Fluidity Manual for indoor-outdoor exchanges and urban environment simulations

The aim of this document is to show how Fluidity can be used to set up typical indoor simulations under a range of conditions. Further information can also be found in the Fluidity manual and online http://fluidityproject.github.io/. The purpose of this document is to allow a new Fluidity user to quickly become independent and start running simulations early on. Despite its length, it should be read carefully and followed step by step. Concrete examples will be used and developed along this document, all sections being equally important. In addition, the tricks and information given might be directly experience based and as such might not appear in the Fluidity manual.

==> 0_Test.tex <==
\chapter{Test}

As we can see in Command~\ref{Lst:BuildFluidity} we have a command line, while in Code~\ref{Lst:GeoParameters} and Code~\ref{Lst:PythonMinEdge}, we have a fucking code.

\begin{Terminal}[caption={BLALBIOa hf jsdfh}, label={Lst:BuildFluidity}]
ä\colorbox{davysgrey}{
\parbox{435pt}{
\color{applegreen} \textbf{user@mypc}\color{white}\textbf{:}\color{codeblue}$\sim$
\color{white}\$ sudo cp lib*.a /usr/lib
\newline
\color{applegreen} \textbf{user@mypc}\color{white}\textbf{:}\color{codeblue}$\sim$
\color{white}\$ sudo cp parmetis.h /usr/include
\newline
\color{applegreen} \textbf{user@mypc}\color{white}\textbf{:}\color{codeblue}$\sim$
\color{white}\$ sudo cp lib*.a <<FluiditySourcePath>>/lib
\newline
\color{applegreen} \textbf{user@mypc}\color{white}\textbf{:}\color{codeblue}$\sim$
\color{white}\$ sudo cp parmetis.h <<FluiditySourcePath>>/include
}
}
\end{Terminal}

\begin{Code}[language=C, caption={Parameters defining the geometry - from the \textit{*.geo} file}, label={Lst:GeoParameters}]
//--------------------------------------//
// Parameters defining the geometry     //
//--------------------------------------//
// NB: All the following parameters are used to define the geometry.

//--> Rotation of the geometry
theta = 0.0; // in degree

//--> Elements size (edge length) of the mesh
m_domain_top     = 3.0;
m_domain_bottom  = 0.5;

\end{Code}

\begin{Code}[language=python, caption={Python script to prescribed different minimum edge length in different region used in \textit{3dBox\_Case9b.flml}.}, label={Lst:PythonMinEdge}]
def val(X, t):
  # Function code
  # Geometry variables
  x_source = 9.0 # x-position of the center of the source
  y_source = 9.0 # y-position of the center of the source
  z_source = 0.0 # z-position of the center of the source

  val = [[s_domain,0.0,0.0],[0.0,s_domain,0.0],[0.0,0.0,s_domain]]
  
  if (X[2] >= zmin) and (X[2] <= zmax):
    if (X[1] >= ymin) and (X[1] <= ymax):
      if (X[0] >= xmin) and (X[0] <= xmax):
        val = [[s_source,0.0,0.0],[0.0,s_source,0.0],[0.0,0.0,s_source]]

  return val #Return value
\end{Code}

\begin{Terminal}[caption={BLALBIOa hf jsdfh}, label={Lst:yoyo}]
ä\colorbox{davysgrey}{
\parbox{435pt}{
\color{applegreen} \textbf{user@mypc}\color{white}\textbf{:}\color{codeblue}$\sim$
\color{white}\$ sudo cp lib*.a /usr/lib
\newline
\color{applegreen} \textbf{user@mypc}\color{white}\textbf{:}\color{codeblue}$\sim$
\color{white}\$ sudo cp parmetis.h /usr/include
\newline
\color{applegreen} \textbf{user@mypc}\color{white}\textbf{:}\color{codeblue}$\sim$
\color{white}\$ sudo cp lib*.a <<FluiditySourcePath>>/lib
\newline
\color{applegreen} \textbf{user@mypc}\color{white}\textbf{:}\color{codeblue}$\sim$
\color{white}\$ sudo cp parmetis.h <<FluiditySourcePath>>/include
}
}
\end{Terminal}

\chapter{Test}

As we can see in Command~\ref{Lst:BuildFluidity} we have a command line, while in Code~\ref{Lst:GeoParameters} and Code~\ref{Lst:PythonMinEdge}, we have a fucking code.

\begin{Terminal}[caption={BLALBIOa hf jsdfh}, label={Lst:BuildFluidity}]
ä\colorbox{davysgrey}{
\parbox{435pt}{
\color{applegreen} \textbf{user@mypc}\color{white}\textbf{:}\color{codeblue}$\sim$
\color{white}\$ sudo cp lib*.a /usr/lib
\newline
\color{applegreen} \textbf{user@mypc}\color{white}\textbf{:}\color{codeblue}$\sim$
\color{white}\$ sudo cp parmetis.h /usr/include
\newline
\color{applegreen} \textbf{user@mypc}\color{white}\textbf{:}\color{codeblue}$\sim$
\color{white}\$ sudo cp lib*.a <<FluiditySourcePath>>/lib
\newline
\color{applegreen} \textbf{user@mypc}\color{white}\textbf{:}\color{codeblue}$\sim$
\color{white}\$ sudo cp parmetis.h <<FluiditySourcePath>>/include
}
}
\end{Terminal}

\begin{Code}[language=C, caption={Parameters defining the geometry - from the \textit{*.geo} file}, label={Lst:GeoParameters}]
//--------------------------------------//
// Parameters defining the geometry     //
//--------------------------------------//
// NB: All the following parameters are used to define the geometry.

//--> Rotation of the geometry
theta = 0.0; // in degree

//--> Elements size (edge length) of the mesh
m_domain_top     = 3.0;
m_domain_bottom  = 0.5;

\end{Code}

\begin{Code}[language=python, caption={Python script to prescribed different minimum edge length in different region used in \textit{3dBox\_Case9b.flml}.}, label={Lst:PythonMinEdge}]
def val(X, t):
  # Function code
  # Geometry variables
  x_source = 9.0 # x-position of the center of the source
  y_source = 9.0 # y-position of the center of the source
  z_source = 0.0 # z-position of the center of the source

  val = [[s_domain,0.0,0.0],[0.0,s_domain,0.0],[0.0,0.0,s_domain]]
  
  if (X[2] >= zmin) and (X[2] <= zmax):
    if (X[1] >= ymin) and (X[1] <= ymax):
      if (X[0] >= xmin) and (X[0] <= xmax):
        val = [[s_source,0.0,0.0],[0.0,s_source,0.0],[0.0,0.0,s_source]]

  return val #Return value
\end{Code}

\begin{Terminal}[caption={BLALBIOa hf jsdfh}, label={Lst:yoyo}]
ä\colorbox{davysgrey}{
\parbox{435pt}{
\color{applegreen} \textbf{user@mypc}\color{white}\textbf{:}\color{codeblue}$\sim$
\color{white}\$ sudo cp lib*.a /usr/lib
\newline
\color{applegreen} \textbf{user@mypc}\color{white}\textbf{:}\color{codeblue}$\sim$
\color{white}\$ sudo cp parmetis.h /usr/include
\newline
\color{applegreen} \textbf{user@mypc}\color{white}\textbf{:}\color{codeblue}$\sim$
\color{white}\$ sudo cp lib*.a <<FluiditySourcePath>>/lib
\newline
\color{applegreen} \textbf{user@mypc}\color{white}\textbf{:}\color{codeblue}$\sim$
\color{white}\$ sudo cp parmetis.h <<FluiditySourcePath>>/include
}
}
\end{Terminal}
